Bootstrapping Generalization Error Bounds for Time Series

We consider the problem of finding confidence intervals for the risk of forecasting the future of a stationary, ergodic stochastic process, using a model estimated from the past of the process. We show that a bootstrap procedure provides valid confidence intervals for the risk, when the data source is sufficiently mixing, and the loss function and the estimator are suitably smooth. Autoregressive (AR(d)) models estimated by least squares obey the necessary regularity conditions, even when mis-specified, and simulations show that the finite- sample coverage of our bounds quickly converges to the theoretical, asymptotic level. As an intermediate step, we derive sufficient conditions for asymptotic independence between empirical distribution functions formed by splitting a realization of a stochastic process, of independent interest.

==> summary.tex <==
%Our main contribution  is establishing sufficient conditions for bootstrap %consistency to hold for the generalization error without assuming an explicit form %on the data generating process.   We establish Hadamard differentiability of the %parametric model as the key requirement for the estimator to be ``smooth enough'' %for bootstrap consistency to hold.

%Using our theorem, we show that unconstrained squared error loss estimators are %Hadamard differentiable under weak and relatively simple conditions. As an %intermediate step, we derive sufficient conditions for the joint distribution of the %empirical distributions for the test and training set to converge to a Gaussian %process under weak dependence. In simulations, we study the finite sample properties %of our procedure using AR(p) models for prediction on several geometrically $\beta$-%mixing processes

\begin{itemize}
\item We propose a novel procedure based on the block bootstrap for computing
  confidence intervals for the risk of time series models.  We establish
  bootstrap consistency of an estimator of the generalization error in the weak
  assumption setting, with no assumptions about the functional form of the data
  generating process. The $\beta$-mixing rates we impose are polynomial, which
  are satisfied for a wide range of processes.  To our knowledge, we are the
  first to study the theoretical properties of bootstrapped generalization
  errors in the dependent setting when the model is wrong and the first to
  propose confidence intervals for this term in the dependent setting.
\item We place stronger assumptions on the model used by the data analyst, but
  still show that least squares models meet these conditions when the
  stochastic process is compactly supported.  Therefore, our procedure may be
  used to construct asymptotically valid confidence intervals for the risk of
  $AR(p)$ models, which are very commonly used in practice.
\item We establish sufficient conditions for asymptotic independence of
  empirical processes formed by splitting a stochastic process.  This result
  has implications beyond the current problem.  In particular, for well-behaved
  loss functions and plug-in estimators of $d$-dimensional distributions, the
  Functional Delta Method implies both asymptotic Normality and consistency of
  K-fold cross-validation for the risk even in the dependent setting.
\item We establish sufficient conditions for the equivalence of the conditional
  ergodic risk defined in \citet{CRS-Leo-predictive-mixtures} and a conditional
  risk evaluated on an independent dataset. Therefore, for certain processes,
  generalization along a given realization of a stochastic process is
  equivalent to generalization over different runs of the same process.
\item We examine the finite sample performance of our procedure in a simulation
  study even in cases where the model is badly misspecified and show that we
  still reach the desired coverage level.
\end{itemize}
